Robustness Certification of Generative Models

Generative neural networks can be used to specify continuous transformations between images via latent-space interpolation. However, certifying that all images captured by the resulting path in the image manifold satisfy a given property can be very challenging. This is because this set is highly non-convex, thwarting existing scalable robustness analysis methods, which are often based on convex relaxations. We present ApproxLine, a scalable certification method that successfully verifies non-trivial specifications involving generative models and classifiers. ApproxLine can provide both sound deterministic and probabilistic guarantees, by capturing either infinite non-convex sets of neural network activation vectors or distributions over such sets. We show that ApproxLine is practically useful and can verify interesting interpolations in the networks latent space.

==> approx_line_figure.tex <==
\begin{figure*}[h]
\centering
\begin{tikzpicture}
  \node at (0,0){\includegraphics[width=14cm,trim={0.0cm 0.0cm -0.1cm 0.0cm},clip=true]{images/ApproxLineFig_NoText.pdf}};
  \node[align=center,anchor=center] at (-6,1) {Exact\\Execution};
  \node[align=center,anchor=center] at (-6,-1.1) {\domain{}\\Execution};

  \node[align=center,anchor=center] at (-3.1,1.65) {$n_E$};
  \node[align=center,anchor=center] at (-3.1,0.5) {$n_E$};

  \node[align=center,anchor=center] at (-1.35,0.52) {$\ve_1$};
  \node[align=center,anchor=center] at (-2.05,-0.55) {$\ve_2$};

  \node[align=center,anchor=center] at (-0.05,0.8) {$n_D$};
  \node[align=center,anchor=center] at (-0.04,-1.245) {$n^\#_D$};

  \node[align=center,anchor=center] at (4.56,0.8) {$n_A$};
  \node[align=center,anchor=center] at (4.54,-1.245) {$n^\#_A$};


  \node[align=center,anchor=center, rotate=60] at (-1.95,0.1) {\tiny $\lambda=1$};


  \node[align=center,anchor=center, rotate=0] at (1.125,1.02) {\tiny $.08$}; %
  \node[align=center,anchor=center, rotate=0] at (1.125,-1.18) {\tiny $.08$}; %


  \node[align=center,anchor=center, rotate=-69] at (2.59,1.66) {\tiny $.4$}; %
  \node[align=center,anchor=center, rotate=-69] at (2.59,-0.54) {\tiny $.4$}; %

  \node[align=center,anchor=center, rotate=25.8] at (2.45,0.33) {\tiny $.27$}; %
  \node[align=center,anchor=center, rotate=25.8] at (2.45,-1.87) {\tiny $.27$}; %

  \node[align=center,anchor=center, rotate=0] at (1.8,1.35) {\tiny $.13$}; %
  \node[align=center,anchor=center, rotate=0] at (1.58,-0.65) {\tiny $.13$}; %

  \node[align=center,anchor=center, rotate=0] at (2.28, .75) {\tiny $.12$}; %
  \node[align=center,anchor=center, rotate=0] at (2.16,-1.34) {\tiny $.12$}; %

  \node[align=center,anchor=center, rotate=0] at (5.4,1.75) {\tiny $.13$}; %
  \node[align=center,anchor=center, rotate=0] at (5.6,-0.75) {\tiny $.13$}; %

  \node[align=center,anchor=center, rotate=0] at (6.5,1.05) {\tiny $.05$}; %
  \node[align=center,anchor=center, rotate=0] at (6.15,-1.08) {\tiny $.05$}; %

  \node[align=center,anchor=center, rotate=0] at (5.85,0.25) {\tiny $.12$}; %
  \node[align=center,anchor=center, rotate=0] at (5.85,-1.63) {\tiny $.12$}; %

  \node[align=center,anchor=center, rotate=0] at (6.75,0.3) {\tiny $.07$}; %
  \node[align=center,anchor=center, rotate=0] at (6.64,-1.55) {\tiny $.07$}; %

  \node[align=center,anchor=center, rotate=-28] at (6.45,1.76) {\tiny $.35$}; %
  \node[align=center,anchor=center, rotate=-28] at (6.45,-0.44) {\tiny $.35$}; %

  \node[align=center,anchor=center, rotate=0] at (5.35,0.4) {\tiny $.08$}; %
  \node[align=center,anchor=center, rotate=0] at (5.35,-1.8) {\tiny $.08$}; %

  \node[align=center,anchor=center, rotate=0] at (6.25,0.2) {\tiny $.2$}; %
  \node[align=center,anchor=center, rotate=0] at (6.25,-2) {\tiny $.2$}; %
\end{tikzpicture}
\caption{Using \domain{} to find probability bounds for a generative specification over flipped images.
Green polygonal chains represent activation distributions at each layer exactly. 
Blue boxes are relaxations of segments highlighted by yellow boxes.
We label regions with their probabilities.
}

\label{abstract_example}
\end{figure*}



==> contribution.tex <==


\input{abstraction}

\input{probabilistic}

